Soft Rasterizer: A Differentiable Renderer for Image-based 3D Reasoning

Rendering bridges the gap between 2D vision and 3D scenes by simulating the physical process of image formation. By inverting such renderer, one can think of a learning approach to infer 3D information from 2D images. However, standard graphics renderers involve a fundamental discretization step called rasterization, which prevents the rendering process to be differentiable, hence able to be learned. Unlike the state-of-the-art differentiable renderers, which only approximate the rendering gradient in the back propagation, we propose a truly differentiable rendering framework that is able to (1) directly render colorized mesh using differentiable functions and (2) back-propagate efficient supervision signals to mesh vertices and their attributes from various forms of image representations, including silhouette, shading and color images. The key to our framework is a novel formulation that views rendering as an aggregation function that fuses the probabilistic contributions of all mesh triangles with respect to the rendered pixels. Such formulation enables our framework to flow gradients to the occluded and far-range vertices, which cannot be achieved by the previous state-of-the-arts. We show that by using the proposed renderer, one can achieve significant improvement in 3D unsupervised single-view reconstruction both qualitatively and quantitatively. Experiments also demonstrate that our approach is able to handle the challenging tasks in image-based shape fitting, which remain nontrivial to existing differentiable renderers.

==> fig_color.tex <==
%\begin{figure}[t]
%	\begin{subfigure}[b]{.24\linewidth}
%		\centering
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/chair/input.png}\\
%%		\vspace{-5px}
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/plane/input.png}\\
%		\caption{Input image}
%	\end{subfigure}
%	\begin{subfigure}[b]{.24\linewidth}
%		\centering
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/chair/e+030_a300.png}\\
%%		\vspace{-5px}
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/plane/e+030_a300.png}\\
%		\caption{w/o $\mathcal{L}_{fl}$}
%	\end{subfigure}
%	\begin{subfigure}[b]{.24\linewidth}
%		\centering
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/chair/e+030_a180.png}\\
%%		\vspace{-5px}
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/plane/e+030_a180.png}\\
%%		\caption{w/o $\mathcal{L}_{lap}$}
%	\end{subfigure}
%	\begin{subfigure}[b]{.24\linewidth}
%		\centering
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/chair/e+030_a060.png}\\
%%		\vspace{-5px}
%		\includegraphics[width=\linewidth,trim=66 66 66 66,clip]{render/color/plane/e+030_a060.png}\\
%%		\caption{Full model}
%	\end{subfigure}
%	\caption{Colorized mesh reconstruction. 1st column: input image; 2nd to 4th columns: our reconstructed results.}
%	\label{fig:color}
%\end{figure}



\begin{figure}[t]
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=30 30 30 30,clip]{render/color/chair/input.png}\\
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/color/plane/input.png}\\
		\caption{Input image}
	\end{subfigure}
	\begin{subfigure}[b]{.74\linewidth}
		\centering
		\includegraphics[width=.32\linewidth,trim=40 40 40 40,clip]{render/color/chair/e+030_a300.png}
		\hfill
		\includegraphics[width=.32\linewidth,trim=40 40 40 40,clip]{render/color/chair/e+030_a180.png}
		\hfill
		\includegraphics[width=.32\linewidth,trim=40 40 40 40,clip]{render/color/chair/e+030_a060.png}\\
		
		\includegraphics[width=.32\linewidth,trim=40 40 40 40,clip]{render/color/plane/e+030_a300.png}
		\hfill
		\includegraphics[width=.32\linewidth,trim=40 40 40 40,clip]{render/color/plane/e+030_a180.png}
		\hfill
		\includegraphics[width=.32\linewidth,trim=40 40 40 40,clip]{render/color/plane/e+030_a060.png}\\
		\caption{Reconstruction results}
	\end{subfigure}
	\vspace{-2mm}
	\caption{Results of colorized mesh reconstruction. }
	\label{fig:color}
	\vspace{-3mm}
\end{figure}


==> fig_illu_gradient_flow.tex <==
\begin{figure}[h!]
  	\centering
	\includegraphics[width=1\linewidth]{gradient_flow.pdf}
\caption{Gradient flow}
  	\label{fig:gradientFlow}
\end{figure}



==> fig_res_real_image.tex <==
\begin{figure}[t]
	
	\begin{subfigure}[b]{.24\linewidth}
		\centering
        \includegraphics[width=\linewidth,trim=0 0 0 0,clip]{render/real_img/car_input.png}\\
		\vspace{10pt}
        \includegraphics[width=\linewidth,trim=20 20 20 20,clip]{render/real_img/table_input.png}
%		\vspace{-10px}
		\caption{Input image}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
        \includegraphics[width=\linewidth,trim=0 0 0 0,clip]{render/real_img/car_p2m_e+005_a090.png}\\
		\vspace{10pt}
        \includegraphics[width=\linewidth,trim=20 20 20 20,clip]{render/real_img/table_p3me+010_a150.png}
%		\vspace{-10px}
		\caption{Pixel2Mesh}
	\end{subfigure}
    \begin{subfigure}[b]{.50\linewidth}
		\centering
        \includegraphics[width=.49\linewidth,trim=0 0 0 0,clip]{render/real_img/car_chosen_e+005_a225.png}
        \hfill
        \includegraphics[width=.49\linewidth,trim=0 0 0 0,clip]{render/real_img/car_e+005_a135.png} \\
        \vspace{10pt}
        \includegraphics[width=.49\linewidth,trim=20 20 20 20,clip]{render/real_img/table_chosen_e+014_a060.png}
        \hfill
        \includegraphics[width=.49\linewidth,trim=20 20 20 20,clip]{render/real_img/table_e+014_a330.png} \\
%		\vspace{-10px}
        \caption{SoftRas (ours)}
    \end{subfigure}
%    \vspace{-10px}
	\caption{Comparisons of 3D reconstruction from real images. Our results are shown in two different views. \weikai{remove results of pixel2mesh; add results of warcraft.}}
	\label{fig:vis_real}
	\vspace{-2mm}
\end{figure}

==> fig_res_vis120.tex <==
\begin{figure}[h]
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/input_car.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/input_table.png}\\
		\caption{Input image}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/24_car_e+005_a030.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/24_table_e+010_a300.png}\\
		\label{fig:24view}
		\caption{24 views}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/120_car_e+005_a030.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/120_table_e+010_a300.png}\\
		\label{fig:120view}
		\caption{120 views}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/gt_car_e+005_a120.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation_120/gt_table_e+010_a030.png}\\
		\caption{{\footnotesize Ground Truth}}
	\end{subfigure}
	\caption{Comparison of results reconstructed from different numbers of training views. With more training views, our approach can achieve reconstruction with significantly higher accuracy.}
	\label{fig:vis_120}
	\vspace{-3mm}
\end{figure}


==> fig_res_vis_ablation.tex <==
\begin{figure}[h]
	\vspace{-10pt}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation/input_car.png}\\
		\vspace{-6pt}
		\includegraphics[width=\linewidth,trim=36 36 36 36,clip]{render/ablation/input_bench.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=45 45 45 45,clip]{render/ablation/input_plane.png}\\
		\caption{Input image}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation/lf_car_e+030_a300.png}\\
		\vspace{-6pt}
		\includegraphics[width=\linewidth,trim=36 36 36 36,clip]{render/ablation/lf_bench_e+030_a300.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=45 45 45 45,clip]{render/ablation/lf_plane_e+030_a300.png}\\
		\caption{w/o $\mathcal{L}_{fl}$}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation/ll_car_e+030_a300.png}\\
		\vspace{-6pt}
		\includegraphics[width=\linewidth,trim=36 36 36 36,clip]{render/ablation/ll_bench_e+030_a300.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=45 45 45 45,clip]{render/ablation/ll_plane_e+030_a300.png}\\
		\caption{w/o $\mathcal{L}_{lap}$}
	\end{subfigure}
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=\linewidth,trim=40 40 40 40,clip]{render/ablation/full_car_e+030_a300.png}\\
		\vspace{-6pt}
		\includegraphics[width=\linewidth,trim=36 36 36 36,clip]{render/ablation/full_bench_e+030_a300.png}\\
		\vspace{-10pt}
		\includegraphics[width=\linewidth,trim=45 45 45 45,clip]{render/ablation/full_plane_e+030_a300.png}\\
		\caption{Full model}
	\end{subfigure}
	\vspace{-5pt}
	\caption{Ablation study of different loss terms. \shichen{remove this figure}}
	\label{fig:vis_ablation}
\end{figure}

==> fig_supple_deform_process.tex <==
\begin{figure*}[h]
    \vspace{-10px}
        \includegraphics[width=1.0\linewidth]{supple_deform_process_v1.pdf}
    \vspace{-5px}
    \caption{Demonstration for mesh deformation process while training on only one input image.}
    \label{fig:supple_deform_process}
\end{figure*}

==> fig_supple_more_result.tex <==
\begin{figure*}[t!]
    \vspace{-10px}
    \includegraphics[scale=0.4]{supple_more_result_part_1_v1.png}
    \centering
    \vspace{-5px}
    \caption{More reconstruction results using our approach. Leftmost column: input image; the rest columns: results visualized from multiple viewpoints.}
    \label{fig:supple_more_result_part_1}
\end{figure*}

\begin{figure*}[t!]
    \vspace{-10px}
    \includegraphics[scale=0.4]{supple_more_result_part_2_v1.png}
    \centering
    \vspace{-5px}
    \caption{More reconstruction results using our approach. Leftmost column: input image; the rest columns: results visualized from multiple viewpoints.}
    \label{fig:supple_more_result_part_2}
\end{figure*}

\begin{figure*}[t!]
    \vspace{-10px}
    \includegraphics[scale=0.4]{supple_more_result_part_3_v1.png}
    \centering
    \vspace{-5px}
    \caption{More reconstruction results using our approach. Leftmost column: input image; the rest columns: results visualized from multiple viewpoints.}
    \label{fig:supple_more_result_part_3}
\end{figure*}

==> fig_supple_sigma_gamma.tex <==
\nothing{
\begin{figure*}[tb!]
%    \vspace{-10px}
    \centering
    \includegraphics[width=\textwidth]{supple_sigma_gamma.pdf}
%    \vspace{-5px}
    \caption{Rendering effect of SoftRas with different $\gamma$ and $\sigma$, where $\gamma \rightarrow 0$ and $\sigma \rightarrow 0$ lead to more realistic rendering effect.}
    \label{fig:supple_sigma_gamma}
\end{figure*}
}%nothing

\twocolumn[{%
	\renewcommand\twocolumn[1][]{#1}%
	\maketitle
	\begin{center}
		\centering
		\includegraphics[width=\textwidth]{supple_sigma_gamma}
		\captionof{figure}{Different rendering effects achieved by our proposed SoftRas renderer. We show how a colorized cube can be rendered in various ways by tuning the parameters of SoftRas. In particular, by increasing $\gamma$, SoftRas can render the object with more tranparency while more blurry renderings can be achieved via increasing $\sigma$. As $\gamma \rightarrow 0$ and $\sigma \rightarrow 0$, one can achieve rendering effect closer to standard rendering. 
			%Rendering effect of SoftRas with different $\gamma$ and $\sigma$, where $\gamma \rightarrow 0$ and $\sigma \rightarrow 0$ lead to more realistic rendering effect.
			}
		\label{fig:supple_sigma_gamma}
	\end{center}%
}]

==> pose_estimation.tex <==
\subsection{Pose Estimation}
\label{sec:pose}

==> result_pose.tex <==
\subsection{Pose Estimation}
\label{sec:result_pose}



==> sec_network.tex <==
\section{Network Architecture}
\label{sec:network}




==> suppl_video.tex <==
\section{Video}
\label{sec:suppl_video}

We also include a \textit{supplemental video} that provides animated visualization of our results. 
Please refer to the video for more details. 

%In the \textit{supplemental video}, we show the animated visualization of (1) our forward rendering; (2) more reconstruction results; (3) the mesh deformation procedure and (4) the fitting process of SMPL pose optimization.


==> tab_functions.tex <==
\begin{table}[h!]
\addtolength{\tabcolsep}{4pt}
\centering
\begin{tabular}{ccc}
\hline
bary. + NN   & bary. + Or   & bary. + smoothMax     \\ 
\hline
XXXX   & XXXX  & XXXX \\
\hline
dist. + NN   & dist. + Or   & dist. + smoothMax    \\ \hline
XXXX   & XXXX  & XXXX \\
\hline
\end{tabular}

\vspace{2pt}
\caption{Quantitative results of using different combinations of probability and aggregation functios.}
\label{tab:functions}
\vspace{-5mm}
\end{table}

==> tab_gradient_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{ll|c|c|c}
                                        &          & openDR        & NMR           & SoftRas            \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{U}} & forward  & rasterization & rasterization & Prob map \\ \cline{2-5} 
\multicolumn{1}{l|}{}                   & backward & filter        & linear        & gradient           \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Z}} & forward  & z-buffer      & z-buffer      & aggr func          \\ \cline{2-5} 
\multicolumn{1}{l|}{}                   & backward & none          & none          & gradient           \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{A}} & forward  & vertex color  & face color    & vertex/face               \\ \cline{2-5} 
\multicolumn{1}{c|}{}                   & backward & gradient      & gradient      & gradient          \\ \hline

\end{tabular}
\end{table}
